Refinement Types for Ruby

Refinement types are a popular way to specify and reason about key program properties. In this paper, we introduce RTR, a new system that adds refinement types to Ruby. RTR is built on top of RDL, a Ruby type checker that provides basic type information for the verification process. RTR works by encoding its verification problems into Rosette, a solver-aided host language. RTR handles mixins through assume-guarantee reasoning and uses just-in-time verification for metaprogramming. We formalize RTR by showing a translation from a core, Ruby-like language with refinement types into Rosette. We apply RTR to check a range of functional correctness properties on six Ruby programs. We find that RTR can successfully verify key methods in these programs, taking only a few minutes to perform verification.

==> overview.old.tex <==
\section{Overview}\label{sec:overview}

\begin{figure}[!ht]
\begin{lstlisting}[style=ruby, frame=single]
class Customer
  var_type :@balance, "%integer"
  type "(%integer) (*$\rightarrow$*) %integer"
  def withdraw(amount)
    raise "Insufficient funds." if amount > @balance
    @balance = @balance - amount
  end
  type "(%integer) (*$\rightarrow$*) %integer"
  def deposit(amount)
    @balance = @balance + amount
  end
  type "() (*$\rightarrow$*) %integer"
  def current_balance
    @balance
  end
end

class Bank
  var_type :@log, "Array<%integer>"
  type "(%integer) (*$\rightarrow$*) %bool"
  def self.log_transaction(tid)
    raise "ID is already in log!" if @log.include?(tid)
    @log << tid
    true
  end
  type "(Customer c1, Customer c2, %integer amount {{ c1.current_balance > amount }}, %integer tid) (*$\rightarrow$*) Array<%integer> log {{ log.include?(tid) }}"
  def self.transaction(c1, c2, amount, tid)
    c1.withdraw amount
    c2.deposit amount
    log_transaction tid
    return @log
  end
end
\end{lstlisting}
\caption{Overview the translation from Ruby to Rosette.}
\label{fig:bankexample}
\end{figure}
We begin by presenting a simple Ruby program with refinement types. Figure \ref{fig:bankexample} shows a Ruby program which defines two classes, \code{Customer} and \code{Bank}. \code{Customer} defines three instance methods: \code{withdraw}, which subtracts the given input \code{amount} from the \code{@balance} field or raises an error if the given amount exceeds this field, \code{deposit}, which adds the given input to \code{@balance}, and \code{current\_balance}, which returns the value of \code{@balance}. \code{Bank} defines two class methods: \code{log\_transaction}, which appends a given unique transaction ID to the \code{@log} array field, and \code{transaction}, which takes as input two customers, a specified integer amount, and a unique transaction ID, and performs and logs a transaction between the two customers and finally returning the log. The classes may define other methods, such as constructors, but we only show this subset of methods for simplicity.

We also use RDL to provide a number of type annotations. Preceding every method definition is a type signature. A signature is actually a call to the \code{type} method, which takes a string, parses it into RDL's type system, and stores it in a global table. \code{type} may take additional arguments indicating if and when a method should be type checked or verified; we have again elided this detail for simplicity. RDL also includes extensive type annotations for Ruby's standard and core library methods. Each class in Figure \ref{fig:bankexample} also includes a call to \code{var\_type}, which defines the type of an instance variable.

The type annotation for \code{transaction} on line 26 makes use of refinement types in two places. The input \code{amount} has type Integer with a refinement indicating that \code{amount} must be less than the current balance of customer \code{c1}. This is effectively a precondition on the method. The method output, \texttt{log} is specified to be an Array of Integers, with the refinement that \code{log} must include \code{tid} as an element, the transaction ID provided as an input. This is a post condition on the method.

RDL can dynamically check refinement types over methods, such as the ones specified in Figure \ref{fig:bankexample}. But our refinement type verifier introduces static verification for such refinement types. The verifier assumes refinements on method inputs to be true, and tries to prove the refinement on the output will hold. After attempting to verify a method, we notify the programmer either that their method is safe, or we attempt to provide them with a counter example to their asserted postcondition. The reader may have noticed that the refinement type from Figure \ref{fig:bankexample} will actually fail to verify! This is because if input \code{tid} (the transaction ID) to the \code{transaction} method already exists in \code{@log} (i.e., it is not unique), then the \code{log\_transaction} method will raise an error. Thus, in order to pass the verifier, we need to include an additional refinement on \code{tid} which says that it is not already in the log, or \code{!@log.include?(tid)}. 

Currently, we allow the programmer to insert arbitrary code within type refinements, and we attempt to verify that this refinement always evaluates to \code{true} if it is a method postcondition. Of course, there are limitations as to what can actually be verified. If a predicate asserts some undecidable property, the verifier may diverge or return a result of ``unknown.'' The verifier may also fail if the programmer asserts some property that is not modeled by the verifier. Thus, even though arbitrary code is allowed within refinements, the programmer must use discretion in what assertions they try to verify.

\subsection{Rosette}

We achieve verification of Ruby refinement types by translating Ruby programs and appropriate verification queries to Rosette. Rosette is a language that extends a subset of Racket with constructs for accessing a back-end solver. Specifically, Rosette includes constructs for program synthesis, angelic execution, and verification. In order to achieve verification, Rosette uses symbolic execution to generate logical constraints, and discharges these constraints using \textit{Z3}\cite{deMoura} as its back-end SMT solver.

Shown below is a brief example of a Rosette program with a verification query. Line 1 defines an absolute value function \code{abs\_val}. Line 2 defines an integer \textit{symbolic constant} \code{sym\_x}. We can think of \code{sym\_x} as a placeholder for some concrete integer for which we do not know the value. Rosette allows us to define symbolic constants of what it considers to be \textit{solvable types}: integers, reals, booleans, and uninterpreted functions. Finally, line 3 presents a verification query, in which we attempt to verify the assertion that \code{abs\_val} of \code{sym\_x} is greater than or equal to zero. This assertion is indeed valid, so Rosette will notify us that the negation of this assertion is unsatisfiable. If we attempt to verify an invalid assertion, Rosette will provide us with a model of bindings to symbolic constants such that the assertion fails.

\begin{lstlisting}[style=rosette]
(define (abs_val x) (if (>= x 0) x (- 0 x)))
(define-symbolic sym_x integer?)
(verify (assert (>= (abs_val sym_x) 0)))
\end{lstlisting}


% \section{Translation From Ruby To Rosette}

The translation from Ruby to Rosette is complex for a number of reasons. Ruby is object-oriented, while Rosette is not. Ruby uses dynamic dispatch for method calls, making it difficult to determine how to translate method calls to Rosette. Ruby also includes a number of statements that alter the control flow of a method, for which there are no direct analogs in Rosette. Figure \ref{fig:diagram} provides an overview of the translation process, and the subsequent sections explain how we addressed these translation challenges.

\begin{figure}[h]

\centering
\begin{tikzpicture}
[node distance = 1cm, auto,font=\footnotesize,
% STYLES
every node/.style={node distance=3cm},
comment/.style={rectangle, inner sep= 5pt, text width=1.25cm, node distance=0.25cm, font=\scriptsize\sffamily, text badly centered},
%prog style
prog/.style={rectangle, draw, fill=black!10, inner sep=5pt, text width=1cm, text badly centered, minimum height=3cm, font=\bfseries\scriptsize\sffamily}]

% Draw nodes

\node [prog] (rubyprog) {Ruby Program};

\node [prog, right = 1cm of rubyprog, minimum height=1cm] (methods) {Methods};
\node [prog, above = 0.25 of methods, minimum height=1cm] (fields) {Instance Variables};
\node [prog, below = 0.25 of methods, minimum height=1cm] (spec) {Spec. to Verify};

\node [prog, right = 0.5 of methods, minimum height = 1cm, text width=1.2cm] (typecheck) {Type Checking};

\node [prog, right = 0.5 of typecheck, minimum height = 1cm] (functions) {Function Defs.};
\node [prog, above = 0 of functions, minimum height = 1cm] (struct) {Object Struct Def.};
\node [prog, below = 0 of functions, minimum height = 1cm] (assert) {Assertion};
\node [comment, below = 0 of assert] (IL) {Intermediate Language};

\node [prog, right = 1.5cm of functions] (rosette) {Rosette Program};
\node [comment, right = 1cm of rosette, text width = 1.5cm] (output) {Output to Programmer};

% Draw paths
\path[->,thick] 
(rubyprog) edge (methods)
(rubyprog) edge (fields)
(rubyprog) edge (spec)
(methods) edge (typecheck)
(typecheck) edge (functions)
(fields) edge (struct)
(spec) edge node[comment, below = 0.5] {Translation} (assert)
(functions) edge node[comment, below] {Macro Expansion} (rosette)
(rosette) edge (output)
;

\end{tikzpicture} 
\caption{Overview the translation from Ruby to Rosette.}
\label{fig:diagram}
\end{figure}

\subsection{Encoding Objects}

One issue faced in the translation is that Ruby is object-oriented while Rosette is not. To address this problem, we follow a similar approach to \cite{Jeon} and \cite{Singh}, and encode all Ruby objects using a new \code{object} type defined in Rosette. This \code{object} type is defined using a \code{struct} which contains all fields (instance variables) of all objects encountered in the Ruby program, as well as an integer identifying the object's class, and an integer identifying the object itself. For instance, the program in Figure \ref{fig:bankexample} uses two instance variables: the \code{Customer} class uses the the \code{@balance} variable, and the \code{Bank} class uses the \code{@log} variable. The resulting \code{object} struct definition in Rosette would look as follows:

\begin{lstlisting}[style=rosette]
(struct object
  ([classid]
   [objectid]
   [@balance #:auto #:mutable]
   [@log #:auto #:mutable]
   #:auto-value (void)))
\end{lstlisting}

This defines a struct type with fields \code{classid}, \code{objectid}, \code{@balance}, and \code{@log}. The \code{\#:auto} keyword indicates that the corresponding field will be automatically defined with a default value when a new \code{object} is created, and line 6 sets this default value to be Rosette's \code{void} constant. This corresponds nicely with \code{nil}, Ruby's default value for instance variables. We note that the approach outlined here does not handle reflection, namely the dynamic definition of new object fields, which is allowed in Ruby. Rather, only those fields which are statically evident are included in the translation to Rosette.

It's noteworthy that there are no primitive values in Ruby. All values in Ruby are objects. As such, instead of using Rosette's primitives, we encode Ruby objects such as integers using the \code{object} type in Rosette as well. We simply maintain a \code{value} field in the \code{object} type which contains the Rosette primitive corresponding the Ruby object. In the case of integers, we also include a configuration option determining whether a program's integers will be encoded using Rosette's integers or bitvectors of a specified, finite size. Even though Ruby integers are arbitrary precision, this allows the programmer to bound the size of the encoded integer and thus possibly avoid issues of undecidability for certain programs. 


\subsection{Method Calls}\label{subsec:method-calls}
\subsubsection{Method Dispatch}
The translation of method calls to Rosette poses a number of interesting challenges as well. Foremost among these, because Ruby uses dynamic dispatch, we can't actually statically determine what method is being called. Consider the method \code{deposit} in Figure \ref{fig:bankexample}, which consists of the line \code{@balance = @balance + amount}. Note that because all Ruby values are objects, this amounts to calling \code{@balance}'s \code{+} method, or \code{@balance.+(amount)}. But because we do not statically know the class of \code{x}, we also do not know which \code{+} method is actually being called: in Ruby, it may refer to numeric addition, string concatenation, or array append, among others. Knowing which method is being called is crucial to translating and ultimately verifying such code.

We address this issue by using an approach similar to class hierarchy analysis \cite{Dean}. First, we require the programmer to use RDL's type system to provide a type annotation for any method or instance variable which is to be translated to Rosette. This is why type annotations are included for \textit{all} methods in Figure \ref{fig:bankexample}, not just the method to be verified. Using the provided annotations, we then use RDL to type check the methods, and in the process, we tag each expression in a method AST with its type. During translation to Rosette we can then look up the type of a method call receiver and determine which method we should dispatch to. For the \code{deposit} method of Figure \ref{fig:bankexample}, we would look up the type of \code{@balance}, see it has type Integer, and use this to deduce that \code{+} refers to \code{Integer}'s addition method. The Rosette function resulting from the \code{deposit} method would look as follows:
\begin{lstlisting}[style=rosette]
(define (Customer_inst_withdraw self amount)
  (set-object-@balance! self 
    (Integer_inst_+ (object-@balance self) amount)))
\end{lstlisting}
\code{self} in Ruby is a reserved keyword used to refer to the receiver of a method. It can be thought of as an implicit argument to every method, which we make explicit in every Rosette function, as we have done above. The function name \code{Customer\_inst\_withdraw} follows our naming convention, where \code{Customer} is the name of the method's class, \code{inst} refers to the fact that it's an instance method, and \code{withdraw} refers to the name of the method itself. Reading from or writing to an instance variable in Ruby then amounts to getting or setting the corresponding field of \code{self}; \code{object-@balance} and \code{set-object-@balance} are the relevant getter/setter functions above.

There are some complications in handling method dispatch. For one, we must adapt this approach to handle union types. Consider the following bit of Ruby code:
\begin{lstlisting}[style=ruby]
if (some_condition)
  x = A.new
else
  x = B.new
end
x.foo
\end{lstlisting}

Using the approach we've outlined, during translation we will look up the type of \code{x} on line 6 and find that it has type \code{Union(A, B)}. Given this information, we can't statically know whether to dispatch to \code{A}'s or \code{B}'s instance method \code{foo}.

However, though the type checker is path insensitive, Rosette's symbolic executor will fork and consider each path individually. We can take advantage of this fact, and translate the method call by branching on the class ID of \code{x}. Say, for instance, that \code{A} has class ID 1 and \code{B} has class ID 2. The Rosette code we emit for the method call on line 6 would then look as follows:
\begin{lstlisting}[style=rosette]
(cond [(= (object-classid x) 1) (A_inst_foo x)]
      [(= (object-classid x) 2) (B_inst_foo x)])
\end{lstlisting}

Because the symbolic executor will consider each path of the program individually, it will ``know'' the class ID of \code{x} by the time it reaches this branch, and therefore it can choose the correct corresponding path.

We note that our implementation does not currently handle polymorphic method calls, even though such calls are possible in Ruby. However, the approach outlined above can be extended to handle such calls if we treat the receiver of a method call as having a union type of its own class and all subclasses which define the corresponding method.

\subsubsection{Simulating Method Calls}

If a Ruby method is called from one we wish to verify, then we will typically translate the called method to Rosette as well. However, it is also possible to use a method's type annotation to simulate calling it. There are a number of reasons a user may wish to do this: the called method's code may simply not be available, or the called method may include constructs such as loops which are difficult to statically reason about.

Consider the program below. Here, we wish to translate the method \code{caller}, but it calls \code{no\_code}, a method for which the code is not available. Therefore, the programmer must provide a type annotation for \code{no\_code} so that we can simulate calling it. The annotation, shown on line 5, indicates that \code{no\_code} must take an Integer \code{a} which is greater than 0 and value \code{b} belonging to some class \code{Bar}, and it must return an integer \code{c} such that \code{c} is greater than \code{a}.

\begin{lstlisting}[style=ruby]
def caller(x, y)
  no_code(x+1, y)
end

type :no_code, "(Integer a {{ a>0 }}, Bar b) (*$\rightarrow$*)   Integer c {{ c > a }}"
\end{lstlisting}

We can use this information about \code{no\_code} to simulate its calling. A partial resulting Rosette program is shown below. Lines 2-3 put the arguments into A-normal form \cite{Sabry}, allowing us to specify the order in which the arguments are evaluated, and to more easily refer to the arguments later. We then assert any preconditions on our arguments; in this case on line 6, that \code{a} is greater than 0. Omitted on line 6 is generation of the return value \code{c}, which is discussed in further detail below. Finally, on line 7 we assume our postcondition, and on line 8 we return \code{c}.

\begin{lstlisting}[style=rosette]
(define (caller self x y)
  (let ([a (Integer_inst_+ x (int 1))]
        [b y])
    (begin
       (assert (Integer_inst_> a 0))
       ;;; GENERATE RETURN VALUE c
       (assume (Integer_inst_> c a))
       c)))
\end{lstlisting}

Correctly generating a return value for a method will require more information about the method from the programmer. (cite Dafny here?) The user may add the label \lpure to the annotation for \code{no\_code} indicating that it is a pure method. This tells us two things: (1) given the same input(s), the method will always return the same output, and (2) the method has no side effects. We can represent a pure method using Rosette's uninterpreted functions, which (1) memoize mappings from inputs to outputs, and (2) perform no side effects,  giving us the properties we desire. If we define an uninterpreted function \code{no\_code}, generating a return value \code{c} simply amounts to calling \code{no\_code} on \code{a} and \code{b}. The only complexity here is that Rosette's uninterpreted functions can only operate over solvable types, not arbitrary types such as \code{object}. To get around this, we can use an arbitrary object's unique integer identifier in place of the object itself as an argument to the uninterpreted function.

On the other hand, if a user does not label a method as pure, we assume it to be impure. This means (1) the method may return a different output on different calls with the same input(s), and (2) the method may perform side effects. To simulate (1), we generate a fresh symbolic value for the method's return value. To simulate (2), we allow the user to include a \lprotects label in the method annotation. This label will take a list of arguments to the method which are \textit{not} modified by the method. All method arguments not in this list will have all of their fields replaced by fresh, symbolic values.


==> translation.old.tex <==
% \section{Translation From Ruby To Rosette}

The translation from Ruby to Rosette is complex for a number of reasons. Ruby is object-oriented, while Rosette is not. Ruby uses dynamic dispatch for method calls, making it difficult to determine how to translate method calls to Rosette. Ruby also includes a number of statements that alter the control flow of a method, for which there are no direct analogs in Rosette. Figure \ref{fig:diagram} provides an overview of the translation process, and the subsequent sections explain how we addressed these translation challenges.

\begin{figure}[h]

\centering
\begin{tikzpicture}
[node distance = 1cm, auto,font=\footnotesize,
% STYLES
every node/.style={node distance=3cm},
comment/.style={rectangle, inner sep= 5pt, text width=1.25cm, node distance=0.25cm, font=\scriptsize\sffamily, text badly centered},
%prog style
prog/.style={rectangle, draw, fill=black!10, inner sep=5pt, text width=1cm, text badly centered, minimum height=3cm, font=\bfseries\scriptsize\sffamily}]

% Draw nodes

\node [prog] (rubyprog) {Ruby Program};

\node [prog, right = 1cm of rubyprog, minimum height=1cm] (methods) {Methods};
\node [prog, above = 0.25 of methods, minimum height=1cm] (fields) {Instance Variables};
\node [prog, below = 0.25 of methods, minimum height=1cm] (spec) {Spec. to Verify};

\node [prog, right = 0.5 of methods, minimum height = 1cm, text width=1.2cm] (typecheck) {Type Checking};

\node [prog, right = 0.5 of typecheck, minimum height = 1cm] (functions) {Function Defs.};
\node [prog, above = 0 of functions, minimum height = 1cm] (struct) {Object Struct Def.};
\node [prog, below = 0 of functions, minimum height = 1cm] (assert) {Assertion};
\node [comment, below = 0 of assert] (IL) {Intermediate Language};

\node [prog, right = 1.5cm of functions] (rosette) {Rosette Program};
\node [comment, right = 1cm of rosette, text width = 1.5cm] (output) {Output to Programmer};

% Draw paths
\path[->,thick] 
(rubyprog) edge (methods)
(rubyprog) edge (fields)
(rubyprog) edge (spec)
(methods) edge (typecheck)
(typecheck) edge (functions)
(fields) edge (struct)
(spec) edge node[comment, below = 0.5] {Translation} (assert)
(functions) edge node[comment, below] {Macro Expansion} (rosette)
(rosette) edge (output)
;

\end{tikzpicture} 
\caption{Overview the translation from Ruby to Rosette.}
\label{fig:diagram}
\end{figure}

\subsection{Encoding Objects}

One issue faced in the translation is that Ruby is object-oriented while Rosette is not. To address this problem, we follow a similar approach to \cite{Jeon} and \cite{Singh}, and encode all Ruby objects using a new \code{object} type defined in Rosette. This \code{object} type is defined using a \code{struct} which contains all fields (instance variables) of all objects encountered in the Ruby program, as well as an integer identifying the object's class, and an integer identifying the object itself. For instance, the program in Figure \ref{fig:bankexample} uses two instance variables: the \code{Customer} class uses the the \code{@balance} variable, and the \code{Bank} class uses the \code{@log} variable. The resulting \code{object} struct definition in Rosette would look as follows:

\begin{lstlisting}[style=rosette]
(struct object
  ([classid]
   [objectid]
   [@balance #:auto #:mutable]
   [@log #:auto #:mutable]
   #:auto-value (void)))
\end{lstlisting}

This defines a struct type with fields \code{classid}, \code{objectid}, \code{@balance}, and \code{@log}. The \code{\#:auto} keyword indicates that the corresponding field will be automatically defined with a default value when a new \code{object} is created, and line 6 sets this default value to be Rosette's \code{void} constant. This corresponds nicely with \code{nil}, Ruby's default value for instance variables. We note that the approach outlined here does not handle reflection, namely the dynamic definition of new object fields, which is allowed in Ruby. Rather, only those fields which are statically evident are included in the translation to Rosette.

It's noteworthy that there are no primitive values in Ruby. All values in Ruby are objects. As such, instead of using Rosette's primitives, we encode Ruby objects such as integers using the \code{object} type in Rosette as well. We simply maintain a \code{value} field in the \code{object} type which contains the Rosette primitive corresponding the Ruby object. In the case of integers, we also include a configuration option determining whether a program's integers will be encoded using Rosette's integers or bitvectors of a specified, finite size. Even though Ruby integers are arbitrary precision, this allows the programmer to bound the size of the encoded integer and thus possibly avoid issues of undecidability for certain programs. 


\subsection{Method Calls}
\subsubsection{Method Dispatch}
The translation of method calls to Rosette poses a number of interesting challenges as well. Foremost among these, because Ruby uses dynamic dispatch, we can't actually statically determine what method is being called. Consider the method \code{deposit} in Figure \ref{fig:bankexample}, which consists of the line \code{@balance = @balance + amount}. Note that because all Ruby values are objects, this amounts to calling \code{@balance}'s \code{+} method, or \code{@balance.+(amount)}. But because we do not statically know the class of \code{x}, we also do not know which \code{+} method is actually being called: in Ruby, it may refer to numeric addition, string concatenation, or array append, among others. Knowing which method is being called is crucial to translating and ultimately verifying such code.

We address this issue by using an approach similar to class hierarchy analysis \cite{Dean}. First, we require the programmer to use RDL's type system to provide a type annotation for any method or instance variable which is to be translated to Rosette. This is why type annotations are included for \textit{all} methods in Figure \ref{fig:bankexample}, not just the method to be verified. Using the provided annotations, we then use RDL to type check the methods, and in the process, we tag each expression in a method AST with its type. During translation to Rosette we can then look up the type of a method call receiver and determine which method we should dispatch to. For the \code{deposit} method of Figure \ref{fig:bankexample}, we would look up the type of \code{@balance}, see it has type Integer, and use this to deduce that \code{+} refers to \code{Integer}'s addition method. The Rosette function resulting from the \code{deposit} method would look as follows:
\begin{lstlisting}[style=rosette]
(define (Customer_inst_withdraw self amount)
  (set-object-@balance! self 
    (Integer_inst_+ (object-@balance self) amount)))
\end{lstlisting}
\code{self} in Ruby is a reserved keyword used to refer to the receiver of a method. It can be thought of as an implicit argument to every method, which we make explicit in every Rosette function, as we have done above. The function name \code{Customer\_inst\_withdraw} follows our naming convention, where \code{Customer} is the name of the method's class, \code{inst} refers to the fact that it's an instance method, and \code{withdraw} refers to the name of the method itself. Reading from or writing to an instance variable in Ruby then amounts to getting or setting the corresponding field of \code{self}; \code{object-@balance} and \code{set-object-@balance} are the relevant getter/setter functions above.

There are some complications in handling method dispatch. For one, we must adapt this approach to handle union types. Consider the following bit of Ruby code:
\begin{lstlisting}[style=ruby]
if (some_condition)
  x = A.new
else
  x = B.new
end
x.foo
\end{lstlisting}

Using the approach we've outlined, during translation we will look up the type of \code{x} on line 6 and find that it has type \code{Union(A, B)}. Given this information, we can't statically know whether to dispatch to \code{A}'s or \code{B}'s instance method \code{foo}.

However, though the type checker is path insensitive, Rosette's symbolic executor will fork and consider each path individually. We can take advantage of this fact, and translate the method call by branching on the class ID of \code{x}. Say, for instance, that \code{A} has class ID 1 and \code{B} has class ID 2. The Rosette code we emit for the method call on line 6 would then look as follows:
\begin{lstlisting}[style=rosette]
(cond [(= (object-classid x) 1) (A_inst_foo x)]
      [(= (object-classid x) 2) (B_inst_foo x)])
\end{lstlisting}

Because the symbolic executor will consider each path of the program individually, it will ``know'' the class ID of \code{x} by the time it reaches this branch, and therefore it can choose the correct corresponding path.

We note that our implementation does not currently handle polymorphic method calls, even though such calls are possible in Ruby. However, the approach outlined above can be extended to handle such calls if we treat the receiver of a method call as having a union type of its own class and all subclasses which define the corresponding method.

\subsubsection{Simulating Method Calls}

If a Ruby method is called from one we wish to verify, then we will typically translate the called method to Rosette as well. However, it is also possible to use a method's type annotation to simulate calling it. There are a number of reasons a user may wish to do this: the called method's code may simply not be available, or the called method may include constructs such as loops which are difficult to statically reason about.

Consider the program below. Here, we wish to translate the method \code{caller}, but it calls \code{no\_code}, a method for which the code is not available. Therefore, the programmer must provide a type annotation for \code{no\_code} so that we can simulate calling it. The annotation, shown on line 5, indicates that \code{no\_code} must take an Integer \code{a} which is greater than 0 and value \code{b} belonging to some class \code{Bar}, and it must return an integer \code{c} such that \code{c} is greater than \code{a}. The programmer also sets the \code{modular} flag to true, indicating we wish to perform a modular form of verification whereby we don't use a method's code.

\begin{lstlisting}[style=ruby]
def caller(x, y)
  no_code(x+1, y)
end

type :no_code, "(Integer a {{ a>0 }}, Bar b) (*$\rightarrow$*)   Integer c {{ c > a }}", modular: true
\end{lstlisting}

We can use this information about \code{no\_code} to simulate its calling. A partial resulting Rosette program is shown below. Lines 2-3 put the arguments into A-normal form \cite{Sabry}, allowing us to specify the order in which the arguments are evaluated, and to more easily refer to the arguments later. We then assert any preconditions on our arguments; in this case on line 6, that \code{a} is greater than 0. Omitted on line 6 is generation of the return value \code{c}, which is discussed in further detail below. Finally, on line 7 we assume our postcondition, and on line 8 we return \code{c}.

\begin{lstlisting}[style=rosette]
(define (caller self x y)
  (let ([a (Integer_inst_+ x (int 1))]
        [b y])
    (begin
       (assert (Integer_inst_> a 0))
       ;;; GENERATE RETURN VALUE c
       (assume (Integer_inst_> c a))
       c)))
\end{lstlisting}

Correctly generating a return value for a method will require more information about the method from the programmer. (cite Dafny here?) The user may add \code{pure: true} to the annotation for \code{no\_code} indicating that it is a pure method. This tells us two things: (1) given the same input(s), the method will always return the same output, and (2) the method has no side effects. We can represent a pure method using Rosette's uninterpreted functions, which (1) memoize mappings from inputs to outputs, and (2) perform no side effects,  giving us the properties we desire. If we define an uninterpreted function \code{no\_code}, generating a return vlue \code{c} then simply amounts to calling \code{no\_code} on \code{a} and \code{b}. The only complexity here is that Rosette's uninterpreted functions can only operate over solvable types, not arbitrary types such as \code{object}. To get around this, we can use an arbitrary object's unique integer identifier in place of the object itself as an argument to the uninterpreted function.

On the other hand, if a user does not label a method as pure, we assume it to be impure. This means (1) the method may return a different output on different calls with the same input(s), and (2) the method may perform side effects. To simulate (1), we generate a fresh symbolic value for the method's return value. To simulate (2), we allow the user to include a \code{modifies} clause in the method annotation. This clause will take a hash, mapping argument names to fields of that argument which may be modified by the method. For instance, if argument \code{b} has a field \code{@baz} which may be modified by \code{no\_code}, we can include in its annotation: \code{modifies: \{:b => [:@baz]\}}. We will then generate a fresh symbolic value for every field modified by the method. 

\subsection{Control Flow}

Ruby includes a number of statements which can alter the control flow of a program, for which there are no analogs in Rosette. In order to encode such statements, we first translate Ruby programs to an intermediate language which includes such statements, then use Racket macro expansion to transform the program to Rosette.

One example is Ruby's \code{return} statement, which causes a method to immediately exit and return whatever value is provided, or return \code{nil} if no value is provided. Since there are no such statements in Rosette, we must encode the possibility of multiple exit points from a function. Using macro expansion, for each function we keep track of a local variable \code{ret}, which represents the value to be returned from our function; initially, \code{ret} is set to a special \code{undefined} value. A call to \code{return} is expanded to update \code{ret} to the value to be returned. We also update every statement \textit{stmt} in the function to \code{(unless-done }\textit{stmt}\code{)}. Here, \code{unless-done} is a guard which checks the value of \code{ret}. If it is still \code{undefined} (i.e., \code{return} has not been called) then we proceed with executing \textit{stmt}. On the other hand, if \code{ret} has been defined, then we have already returned a value so we skip over \textit{stmt}. Finally, \code{ret} must be inserted at the end of the function so that it is indeed the value which is returned. The only additional complexity is that every path must be guaranteed to have a return statement, something which is not required of Ruby methods. However, making this transformation to every method is a fairly trivial addition to the translation process. 

We can use macros to encode other statements as well. Exceptions can be implemented in a nearly identical manner as \code{return} statements. The only difference is we must also check every function application to see if an exception is returned, and if so, the current function must also return an exception. There are more Ruby control flow altering statements to be encoded, however we anticipate that a similar use of macro expansion will be able to handle such statements.
